Broadband Finite-Element Impedance Computation for Parasitic Extraction

Parasitic extraction is a powerful tool in the design process of electromechanical devices, specifically as part of workflows that check electromagnetic compatibility. A novel scheme to extract impedances from CAD device models, suitable for a finite element implementation, is derived from Maxwell's equations in differential form. It provides a foundation for parasitic extraction across a broad frequency range and is able to handle inhomogeneous permittivities and permeabilities, making it more flexible than existing integral equation approaches. The approach allows for the automatic treatment of multi-port models of arbitrary conductor geometry without requiring any significant manual user interaction. This is achieved by computing a connecting source current density that supplies current to the model's terminals, whatever their location in the model, subsequently using this current density to compute the electric field, and finally calculating the impedance via a scalar potential. A mandatory low-frequency stabilization scheme is outlined, ensuring a stable evaluation of the model at low frequencies as well. Two quasistatic approximations and the special case of perfect electric conductors are treated theoretically. The magnetoquasistatic approximation is validated against an analytical model in a numerical experiment. Moreover, the intrinsic capability of the method to treat inhomogeneous permittivities and permeabilities is demonstrated with a simple capacitor-coil model including dielectric insulation and magnetic core materials.

==> images/rs_tikz.tex <==
% Commands reference / draw TikZ lines
% after a \addplot in a PGFPlots figure a label \label{leg:snr} can be defined and referenced with
% \protect\plotref{leg:snr}
% source: http://tex.stackexchange.com/questions/65494/
% problem: warnings of Multiple defined labels: tex.stackexchange.com/questions/277583/
\newcommand{\plotref}[1]{\tikzexternaldisable\ref*{#1}\tikzexternalenable}
\newcommand{\pref}[1]{%
  (\protect\plotref{#1})%
}
%
% equations are referenced as 'Glg.~1.11'
\newcommand{\gref}[1]{Glg.~(\ref{#1})}
%
% lines from a TikZ image cannot be referenced, create one
\newcommand{\rline}[1]{%
  (\protect\raisebox{2pt}{\protect\tikz \protect\draw[#1](0,0) -- (6mm,0);})%
}
%
% Define the Uni Ulm colors
\definecolor{uniblue}{RGB}{125,154,170}
\definecolor{unired}{RGB}{163,38,56}
%
\tikzset{%
    % arrow shape: stealth, latex
    >=stealth,
    %
    %% flow charts
    % -> rectangle blue
    fcrecb/.style={rectangle, rounded corners, align=center, draw=blue, fill=blue!15},
    % -> ellipse red
    fcelr/.style={ellipse, align = center, draw=red, fill=red!20},
    % -> use in document as
    % \tikzset{%
    %   fcblock/.style={fcrecb, minimum width=4cm, minimum height=1.25cm},
    %   fcdecision/.style={fcelr, minimum width=6cm, minimum height=1.25cm},
    % }
    antrsTop/.style 2 args = {antenna, color=#2, yscale=0.5, xscale=0.6, label={[#2,label distance=1.1cm]90:#1}},
    antrsTop/.default={}{black},
    antrsBot/.style 2 args = {antenna, color=#2, yscale=0.5, xscale=0.6, label={[#2,label distance=0cm]-90:#1}},
    antrsBot/.default={}{black},
}


\definecolor{solids1}{RGB}{228,26,28}
\definecolor{solids2}{RGB}{55,126,184}
\definecolor{solids3}{RGB}{77,175,74}
\definecolor{solids4}{RGB}{152,78,163}
\definecolor{solids5}{RGB}{255,127,0}
\definecolor{solids6}{RGB}{255,255,51}
\definecolor{solids7}{RGB}{166,86,40}
\definecolor{solids8}{RGB}{247,129,191}
\definecolor{solids9}{RGB}{153,153,153}

\pgfplotscreateplotcyclelist{solids}{
	{solids1, solid, line width=1pt, mark=o, mark options={solid}},
	{solids2, solid, line width=1pt, mark=triangle, mark options={solid}},
	{solids3, solid, line width=1pt, mark=square, mark options={solid}},
	{solids4, solid, line width=1pt, mark=x, mark options={solid}},
	{solids5, solid, line width=1pt, mark=+, mark options={solid}},
	{solids6, solid, line width=1pt, mark=Mercedes star, mark options={solid}},
	{solids7, solid, line width=1pt, mark=x, mark options={solid}},
	{solids8, solid, line width=1pt, mark=x, mark options={solid}},
	{solids9, solid, line width=1pt, mark=x, mark options={solid}}
}

\pgfplotscreateplotcyclelist{blacks}{%
	{black, solid, thick, mark=x, mark options={solid}},
	{black, densely dashed, thick, mark=o, mark options={solid}},
	{black, densely dashdotted, thick, mark=triangle, mark options={solid}},
	{black, densely dotted, thick, mark=square, mark options={solid}},
	{black, loosely dashed, thick, mark=Mercedes star, mark options={solid}},
}
%
%
% Define the parula colormap
\pgfplotsset{% http://tex.stackexchange.com/questions/228197/
  colormap/parula/.style={%
    colormap={parula}{%
      rgb = (0.2081,0.1663,0.5292)
      rgb = (0.2116,0.1898,0.5777)
      rgb = (0.2123,0.2138,0.627)
      rgb = (0.2081,0.2386,0.6771)
      rgb = (0.1959,0.2645,0.7279)
      rgb = (0.1707,0.2919,0.7792)
      rgb = (0.1253,0.3242,0.8303)
      rgb = (0.0591,0.3598,0.8683)
      rgb = (0.0117,0.3875,0.882)
      rgb = (0.006,0.4086,0.8828)
      rgb = (0.0165,0.4266,0.8786)
      rgb = (0.0329,0.443,0.872)
      rgb = (0.0498,0.4586,0.8641)
      rgb = (0.0629,0.4737,0.8554)
      rgb = (0.0723,0.4887,0.8467)
      rgb = (0.0779,0.504,0.8384)
      rgb = (0.0793,0.52,0.8312)
      rgb = (0.0749,0.5375,0.8263)
      rgb = (0.0641,0.557,0.824)
      rgb = (0.0488,0.5772,0.8228)
      rgb = (0.0343,0.5966,0.8199)
      rgb = (0.0265,0.6137,0.8135)
      rgb = (0.0239,0.6287,0.8038)
      rgb = (0.0231,0.6418,0.7913)
      rgb = (0.0228,0.6535,0.7768)
      rgb = (0.0267,0.6642,0.7607)
      rgb = (0.0384,0.6743,0.7436)
      rgb = (0.059,0.6838,0.7254)
      rgb = (0.0843,0.6928,0.7062)
      rgb = (0.1133,0.7015,0.6859)
      rgb = (0.1453,0.7098,0.6646)
      rgb = (0.1801,0.7177,0.6424)
      rgb = (0.2178,0.725,0.6193)
      rgb = (0.2586,0.7317,0.5954)
      rgb = (0.3022,0.7376,0.5712)
      rgb = (0.3482,0.7424,0.5473)
      rgb = (0.3953,0.7459,0.5244)
      rgb = (0.442,0.7481,0.5033)
      rgb = (0.4871,0.7491,0.484)
      rgb = (0.53,0.7491,0.4661)
      rgb = (0.5709,0.7485,0.4494)
      rgb = (0.6099,0.7473,0.4337)
      rgb = (0.6473,0.7456,0.4188)
      rgb = (0.6834,0.7435,0.4044)
      rgb = (0.7184,0.7411,0.3905)
      rgb = (0.7525,0.7384,0.3768)
      rgb = (0.7858,0.7356,0.3633)
      rgb = (0.8185,0.7327,0.3498)
      rgb = (0.8507,0.7299,0.336)
      rgb = (0.8824,0.7274,0.3217)
      rgb = (0.9139,0.7258,0.3063)
      rgb = (0.945,0.7261,0.2886)
      rgb = (0.9739,0.7314,0.2666)
      rgb = (0.9938,0.7455,0.2403)
      rgb = (0.999,0.7653,0.2164)
      rgb = (0.9955,0.7861,0.1967)
      rgb = (0.988,0.8066,0.1794)
      rgb = (0.9789,0.8271,0.1633)
      rgb = (0.9697,0.8481,0.1475)
      rgb = (0.9626,0.8705,0.1309)
      rgb = (0.9589,0.8949,0.1132)
      rgb = (0.9598,0.9218,0.0948)
      rgb = (0.9661,0.9514,0.0755)
      rgb = (0.9763,0.9831,0.0538)
    }
  },
  colormap/parula,
}

\pgfplotsset{%
  colormap/hijet/.style={%
    colormap={hijet}{%
      rgb = (0.000000,0.000000,0.562500)
      rgb = (0.000000,0.000000,0.625000)
      rgb = (0.000000,0.000000,0.687500)
      rgb = (0.000000,0.000000,0.750000)
      rgb = (0.000000,0.000000,0.812500)
      rgb = (0.000000,0.000000,0.875000)
      rgb = (0.000000,0.000000,0.937500)
      rgb = (0.000000,0.000000,1.000000)
      rgb = (0.000000,0.062500,1.000000)
      rgb = (0.000000,0.125000,1.000000)
      rgb = (0.000000,0.187500,1.000000)
      rgb = (0.000000,0.250000,1.000000)
      rgb = (0.000000,0.312500,1.000000)
      rgb = (0.000000,0.375000,1.000000)
      rgb = (0.000000,0.437500,1.000000)
      rgb = (0.000000,0.500000,1.000000)
      rgb = (0.000000,0.562500,1.000000)
      rgb = (0.000000,0.625000,1.000000)
      rgb = (0.000000,0.687500,1.000000)
      rgb = (0.000000,0.750000,1.000000)
      rgb = (0.000000,0.812500,1.000000)
      rgb = (0.000000,0.875000,1.000000)
      rgb = (0.000000,0.937500,1.000000)
      rgb = (0.000000,1.000000,1.000000)
      rgb = (0.062500,1.000000,0.937500)
      rgb = (0.125000,1.000000,0.875000)
      rgb = (0.187500,1.000000,0.812500)
      rgb = (0.250000,1.000000,0.750000)
      rgb = (0.312500,1.000000,0.687500)
      rgb = (0.375000,1.000000,0.625000)
      rgb = (0.437500,1.000000,0.562500)
      rgb = (0.500000,1.000000,0.500000)
      rgb = (0.562500,1.000000,0.437500)
      rgb = (0.625000,1.000000,0.375000)
      rgb = (0.687500,1.000000,0.312500)
      rgb = (0.750000,1.000000,0.250000)
      rgb = (0.812500,1.000000,0.187500)
      rgb = (0.875000,1.000000,0.125000)
      rgb = (0.937500,1.000000,0.062500)
      rgb = (1.000000,1.000000,0.000000)
      rgb = (1.000000,0.937500,0.000000)
      rgb = (1.000000,0.875000,0.000000)
      rgb = (1.000000,0.812500,0.000000)
      rgb = (1.000000,0.750000,0.000000)
      rgb = (1.000000,0.687500,0.000000)
      rgb = (1.000000,0.625000,0.000000)
      rgb = (1.000000,0.562500,0.000000)
      rgb = (1.000000,0.500000,0.000000)
      rgb = (1.000000,0.437500,0.000000)
      rgb = (1.000000,0.375000,0.000000)
      rgb = (1.000000,0.312500,0.000000)
      rgb = (1.000000,0.250000,0.000000)
      rgb = (1.000000,0.187500,0.000000)
      rgb = (1.000000,0.125000,0.000000)
      rgb = (1.000000,0.062500,0.000000)
      rgb = (1.000000,0.000000,0.000000)
      rgb = (0.937500,0.000000,0.000000)
      rgb = (0.875000,0.000000,0.000000)
      rgb = (0.812500,0.000000,0.000000)
      rgb = (0.750000,0.000000,0.000000)
      rgb = (0.687500,0.000000,0.000000)
      rgb = (0.625000,0.000000,0.000000)
      rgb = (0.562500,0.000000,0.000000)
      rgb = (0.500000,0.000000,0.000000)
    }
  },
  colormap/hijet,
}
\pgfplotsset{%
  colormap/hiviridis/.style={%
    colormap={hiviridis}{%
      rgb = (0.267004,0.004874,0.329415)
      rgb = (0.268510,0.009605,0.335427)
      rgb = (0.269944,0.014625,0.341379)
      rgb = (0.271305,0.019942,0.347269)
      rgb = (0.272594,0.025563,0.353093)
      rgb = (0.273809,0.031497,0.358853)
      rgb = (0.274952,0.037752,0.364543)
      rgb = (0.276022,0.044167,0.370164)
      rgb = (0.277018,0.050344,0.375715)
      rgb = (0.277941,0.056324,0.381191)
      rgb = (0.278791,0.062145,0.386592)
      rgb = (0.279566,0.067836,0.391917)
      rgb = (0.280267,0.073417,0.397163)
      rgb = (0.280894,0.078907,0.402329)
      rgb = (0.281446,0.084320,0.407414)
      rgb = (0.281924,0.089666,0.412415)
      rgb = (0.282327,0.094955,0.417331)
      rgb = (0.282656,0.100196,0.422160)
      rgb = (0.282910,0.105393,0.426902)
      rgb = (0.283091,0.110553,0.431554)
      rgb = (0.283197,0.115680,0.436115)
      rgb = (0.283229,0.120777,0.440584)
      rgb = (0.283187,0.125848,0.444960)
      rgb = (0.283072,0.130895,0.449241)
      rgb = (0.282884,0.135920,0.453427)
      rgb = (0.282623,0.140926,0.457517)
      rgb = (0.282290,0.145912,0.461510)
      rgb = (0.281887,0.150881,0.465405)
      rgb = (0.281412,0.155834,0.469201)
      rgb = (0.280868,0.160771,0.472899)
      rgb = (0.280255,0.165693,0.476498)
      rgb = (0.279574,0.170599,0.479997)
      rgb = (0.278826,0.175490,0.483397)
      rgb = (0.278012,0.180367,0.486697)
      rgb = (0.277134,0.185228,0.489898)
      rgb = (0.276194,0.190074,0.493001)
      rgb = (0.275191,0.194905,0.496005)
      rgb = (0.274128,0.199721,0.498911)
      rgb = (0.273006,0.204520,0.501721)
      rgb = (0.271828,0.209303,0.504434)
      rgb = (0.270595,0.214069,0.507052)
      rgb = (0.269308,0.218818,0.509577)
      rgb = (0.267968,0.223549,0.512008)
      rgb = (0.266580,0.228262,0.514349)
      rgb = (0.265145,0.232956,0.516599)
      rgb = (0.263663,0.237631,0.518762)
      rgb = (0.262138,0.242286,0.520837)
      rgb = (0.260571,0.246922,0.522828)
      rgb = (0.258965,0.251537,0.524736)
      rgb = (0.257322,0.256130,0.526563)
      rgb = (0.255645,0.260703,0.528312)
      rgb = (0.253935,0.265254,0.529983)
      rgb = (0.252194,0.269783,0.531579)
      rgb = (0.250425,0.274290,0.533103)
      rgb = (0.248629,0.278775,0.534556)
      rgb = (0.246811,0.283237,0.535941)
      rgb = (0.244972,0.287675,0.537260)
      rgb = (0.243113,0.292092,0.538516)
      rgb = (0.241237,0.296485,0.539709)
      rgb = (0.239346,0.300855,0.540844)
      rgb = (0.237441,0.305202,0.541921)
      rgb = (0.235526,0.309527,0.542944)
      rgb = (0.233603,0.313828,0.543914)
      rgb = (0.231674,0.318106,0.544834)
      rgb = (0.229739,0.322361,0.545706)
      rgb = (0.227802,0.326594,0.546532)
      rgb = (0.225863,0.330805,0.547314)
      rgb = (0.223925,0.334994,0.548053)
      rgb = (0.221989,0.339161,0.548752)
      rgb = (0.220057,0.343307,0.549413)
      rgb = (0.218130,0.347432,0.550038)
      rgb = (0.216210,0.351535,0.550627)
      rgb = (0.214298,0.355619,0.551184)
      rgb = (0.212395,0.359683,0.551710)
      rgb = (0.210503,0.363727,0.552206)
      rgb = (0.208623,0.367752,0.552675)
      rgb = (0.206756,0.371758,0.553117)
      rgb = (0.204903,0.375746,0.553533)
      rgb = (0.203063,0.379716,0.553925)
      rgb = (0.201239,0.383670,0.554294)
      rgb = (0.199430,0.387607,0.554642)
      rgb = (0.197636,0.391528,0.554969)
      rgb = (0.195860,0.395433,0.555276)
      rgb = (0.194100,0.399323,0.555565)
      rgb = (0.192357,0.403199,0.555836)
      rgb = (0.190631,0.407061,0.556089)
      rgb = (0.188923,0.410910,0.556326)
      rgb = (0.187231,0.414746,0.556547)
      rgb = (0.185556,0.418570,0.556753)
      rgb = (0.183898,0.422383,0.556944)
      rgb = (0.182256,0.426184,0.557120)
      rgb = (0.180629,0.429975,0.557282)
      rgb = (0.179019,0.433756,0.557430)
      rgb = (0.177423,0.437527,0.557565)
      rgb = (0.175841,0.441290,0.557685)
      rgb = (0.174274,0.445044,0.557792)
      rgb = (0.172719,0.448791,0.557885)
      rgb = (0.171176,0.452530,0.557965)
      rgb = (0.169646,0.456262,0.558030)
      rgb = (0.168126,0.459988,0.558082)
      rgb = (0.166617,0.463708,0.558119)
      rgb = (0.165117,0.467423,0.558141)
      rgb = (0.163625,0.471133,0.558148)
      rgb = (0.162142,0.474838,0.558140)
      rgb = (0.160665,0.478540,0.558115)
      rgb = (0.159194,0.482237,0.558073)
      rgb = (0.157729,0.485932,0.558013)
      rgb = (0.156270,0.489624,0.557936)
      rgb = (0.154815,0.493313,0.557840)
      rgb = (0.153364,0.497000,0.557724)
      rgb = (0.151918,0.500685,0.557587)
      rgb = (0.150476,0.504369,0.557430)
      rgb = (0.149039,0.508051,0.557250)
      rgb = (0.147607,0.511733,0.557049)
      rgb = (0.146180,0.515413,0.556823)
      rgb = (0.144759,0.519093,0.556572)
      rgb = (0.143343,0.522773,0.556295)
      rgb = (0.141935,0.526453,0.555991)
      rgb = (0.140536,0.530132,0.555659)
      rgb = (0.139147,0.533812,0.555298)
      rgb = (0.137770,0.537492,0.554906)
      rgb = (0.136408,0.541173,0.554483)
      rgb = (0.135066,0.544853,0.554029)
      rgb = (0.133743,0.548535,0.553541)
      rgb = (0.132444,0.552216,0.553018)
      rgb = (0.131172,0.555899,0.552459)
      rgb = (0.129933,0.559582,0.551864)
      rgb = (0.128729,0.563265,0.551229)
      rgb = (0.127568,0.566949,0.550556)
      rgb = (0.126453,0.570633,0.549841)
      rgb = (0.125394,0.574318,0.549086)
      rgb = (0.124395,0.578002,0.548287)
      rgb = (0.123463,0.581687,0.547445)
      rgb = (0.122606,0.585371,0.546557)
      rgb = (0.121831,0.589055,0.545623)
      rgb = (0.121148,0.592739,0.544641)
      rgb = (0.120565,0.596422,0.543611)
      rgb = (0.120092,0.600104,0.542530)
      rgb = (0.119738,0.603785,0.541400)
      rgb = (0.119512,0.607464,0.540218)
      rgb = (0.119423,0.611141,0.538982)
      rgb = (0.119483,0.614817,0.537692)
      rgb = (0.119699,0.618490,0.536347)
      rgb = (0.120081,0.622161,0.534946)
      rgb = (0.120638,0.625828,0.533488)
      rgb = (0.121380,0.629492,0.531973)
      rgb = (0.122312,0.633153,0.530398)
      rgb = (0.123444,0.636809,0.528763)
      rgb = (0.124780,0.640461,0.527068)
      rgb = (0.126326,0.644107,0.525311)
      rgb = (0.128087,0.647749,0.523491)
      rgb = (0.130067,0.651384,0.521608)
      rgb = (0.132268,0.655014,0.519661)
      rgb = (0.134692,0.658636,0.517649)
      rgb = (0.137339,0.662252,0.515571)
      rgb = (0.140210,0.665859,0.513427)
      rgb = (0.143303,0.669459,0.511215)
      rgb = (0.146616,0.673050,0.508936)
      rgb = (0.150148,0.676631,0.506589)
      rgb = (0.153894,0.680203,0.504172)
      rgb = (0.157851,0.683765,0.501686)
      rgb = (0.162016,0.687316,0.499129)
      rgb = (0.166383,0.690856,0.496502)
      rgb = (0.170948,0.694384,0.493803)
      rgb = (0.175707,0.697900,0.491033)
      rgb = (0.180653,0.701402,0.488189)
      rgb = (0.185783,0.704891,0.485273)
      rgb = (0.191090,0.708366,0.482284)
      rgb = (0.196571,0.711827,0.479221)
      rgb = (0.202219,0.715272,0.476084)
      rgb = (0.208030,0.718701,0.472873)
      rgb = (0.214000,0.722114,0.469588)
      rgb = (0.220124,0.725509,0.466226)
      rgb = (0.226397,0.728888,0.462789)
      rgb = (0.232815,0.732247,0.459277)
      rgb = (0.239374,0.735588,0.455688)
      rgb = (0.246070,0.738910,0.452024)
      rgb = (0.252899,0.742211,0.448284)
      rgb = (0.259857,0.745492,0.444467)
      rgb = (0.266941,0.748751,0.440573)
      rgb = (0.274149,0.751988,0.436601)
      rgb = (0.281477,0.755203,0.432552)
      rgb = (0.288921,0.758394,0.428426)
      rgb = (0.296479,0.761561,0.424223)
      rgb = (0.304148,0.764704,0.419943)
      rgb = (0.311925,0.767822,0.415586)
      rgb = (0.319809,0.770914,0.411152)
      rgb = (0.327796,0.773980,0.406640)
      rgb = (0.335885,0.777018,0.402049)
      rgb = (0.344074,0.780029,0.397381)
      rgb = (0.352360,0.783011,0.392636)
      rgb = (0.360741,0.785964,0.387814)
      rgb = (0.369214,0.788888,0.382914)
      rgb = (0.377779,0.791781,0.377939)
      rgb = (0.386433,0.794644,0.372886)
      rgb = (0.395174,0.797475,0.367757)
      rgb = (0.404001,0.800275,0.362552)
      rgb = (0.412913,0.803041,0.357269)
      rgb = (0.421908,0.805774,0.351910)
      rgb = (0.430983,0.808473,0.346476)
      rgb = (0.440137,0.811138,0.340967)
      rgb = (0.449368,0.813768,0.335384)
      rgb = (0.458674,0.816363,0.329727)
      rgb = (0.468053,0.818921,0.323998)
      rgb = (0.477504,0.821444,0.318195)
      rgb = (0.487026,0.823929,0.312321)
      rgb = (0.496615,0.826376,0.306377)
      rgb = (0.506271,0.828786,0.300362)
      rgb = (0.515992,0.831158,0.294279)
      rgb = (0.525776,0.833491,0.288127)
      rgb = (0.535621,0.835785,0.281908)
      rgb = (0.545524,0.838039,0.275626)
      rgb = (0.555484,0.840254,0.269281)
      rgb = (0.565498,0.842430,0.262877)
      rgb = (0.575563,0.844566,0.256415)
      rgb = (0.585678,0.846661,0.249897)
      rgb = (0.595839,0.848717,0.243329)
      rgb = (0.606045,0.850733,0.236712)
      rgb = (0.616293,0.852709,0.230052)
      rgb = (0.626579,0.854645,0.223353)
      rgb = (0.636902,0.856542,0.216620)
      rgb = (0.647257,0.858400,0.209861)
      rgb = (0.657642,0.860219,0.203082)
      rgb = (0.668054,0.861999,0.196293)
      rgb = (0.678489,0.863742,0.189503)
      rgb = (0.688944,0.865448,0.182725)
      rgb = (0.699415,0.867117,0.175971)
      rgb = (0.709898,0.868751,0.169257)
      rgb = (0.720391,0.870350,0.162603)
      rgb = (0.730889,0.871916,0.156029)
      rgb = (0.741388,0.873449,0.149561)
      rgb = (0.751884,0.874951,0.143228)
      rgb = (0.762373,0.876424,0.137064)
      rgb = (0.772852,0.877868,0.131109)
      rgb = (0.783315,0.879285,0.125405)
      rgb = (0.793760,0.880678,0.120005)
      rgb = (0.804182,0.882046,0.114965)
      rgb = (0.814576,0.883393,0.110347)
      rgb = (0.824940,0.884720,0.106217)
      rgb = (0.835270,0.886029,0.102646)
      rgb = (0.845561,0.887322,0.099702)
      rgb = (0.855810,0.888601,0.097452)
      rgb = (0.866013,0.889868,0.095953)
      rgb = (0.876168,0.891125,0.095250)
      rgb = (0.886271,0.892374,0.095374)
      rgb = (0.896320,0.893616,0.096335)
      rgb = (0.906311,0.894855,0.098125)
      rgb = (0.916242,0.896091,0.100717)
      rgb = (0.926106,0.897330,0.104071)
      rgb = (0.935904,0.898570,0.108131)
      rgb = (0.945636,0.899815,0.112838)
      rgb = (0.955300,0.901065,0.118128)
      rgb = (0.964894,0.902323,0.123941)
      rgb = (0.974417,0.903590,0.130215)
      rgb = (0.983868,0.904867,0.136897)
      rgb = (0.993248,0.906157,0.143936)
    }
  },
  colormap/hiviridis,
}

